Quantifying point cloud realism through adversarially learned latent representations

Judging the quality of samples synthesized by generative models can be tedious and time consuming, especially for complex data structures, such as point clouds. This paper presents a novel approach to quantify the realism of local regions in LiDAR point clouds. Relevant features are learned from real-world and synthetic point clouds by training on a proxy classification task. Inspired by fair networks, we use an adversarial technique to discourage the encoding of dataset-specific information. The resulting metric can assign a quality score to samples without requiring any task specific annotations. In a series of experiments, we confirm the soundness of our metric by applying it in controllable task setups and on unseen data. Additional experiments show reliable interpolation capabilities of the metric between data with varying degree of realism. As one important application, we demonstrate how the local realism score can be used for anomaly detection in point clouds.

==> paper_figures/experiments_failure_cases.tex <==
% !TEX root = ../paper.tex
%%
\begin{figure}
	\centering

	\begin{tabular}{lll}
		\textcolor{real_img}{\rule{2.4mm}{2.4mm}} \Real{} & \textcolor{syn_img}{\rule{2.4mm}{2.4mm}} \Syn{} & \textcolor{misc_img}{\rule{2.4mm}{2.4mm}} \Misc{}
	\end{tabular}

	\begin{subfigure}{0.48\linewidth}
		\centering

		\begin{tikzpicture}
			\begin{axis}[
				width=1.35\linewidth,
				enlargelimits=false,
				axis on top,
				axis equal image,
				ticks=none,
			]

				\addplot graphics[xmin=-60,xmax=60,ymin=-40,ymax=40] {experiments_anomaly_pandaset_patch_invalid.png};

				\draw[dashed] (0,0) -- (-24,40);
				\draw[dashed] (0,0) -- (-44,-40);

				\addplot graphics[xmin=-2.66,xmax=2.66,ymin=-1.4,ymax=1.4] {ego_vehicle_top_view_ortho.png};

			\end{axis}
		\end{tikzpicture}

		\caption{\label{fig:experiments_failure_cases_invalid}90\% of information loss}
	\end{subfigure}%
	\hspace{4pt}%
	\begin{subfigure}{0.48\linewidth}
		\centering

		\begin{tikzpicture}
			\begin{axis}[
				width=1.35\linewidth,
				enlargelimits=false,
				axis on top,
				axis equal image,
				ticks=none,
			]

				\addplot graphics[xmin=-60,xmax=60,ymin=-40,ymax=40] {experiments_anomaly_pandaset_sensor_failure_512.png};

				\fill[white,opacity=0.6] (0,0) -- (26,-40) -- (-60,-40) -- (-60,-23) -- (0,0);
				\draw[dashed] (0,0) -- (-60,-23);
				\draw[dashed] (0,0) -- (26,-40);

				\addplot graphics[xmin=-2.66,xmax=2.66,ymin=-1.4,ymax=1.4] {ego_vehicle_top_view_ortho.png};

			\end{axis}
		\end{tikzpicture}

		\caption{\label{fig:experiments_failure_cases_failure}Simulated Package Drop}
	\end{subfigure}

	\caption{
		\textbf{Failure Cases}:
		Shown are two examples where we dropped measurements before metric computation (range indicated by dashed lines).
		In (\subref{fig:experiments_failure_cases_invalid}) 90\% of the measurement points are dropped in the respective angle range.
		In (\subref{fig:experiments_failure_cases_failure}) a package drop is simulated, where all measurements in consecutive columns are lost.
		In both cases our metric successfully determines the realism of the scan in regions that are not effected by the augmentations.
		Since our metric cannot determine the realism where there are no points, the metric is not sensitive to inputs that are not full $360^{\circ}$ scans of a point cloud, therefore a package drop remains undetected, see~(\subref{fig:experiments_failure_cases_failure}).
		In the case of information loss, the metric tends to lower its realism score in the sparse regions, see left part of~(\subref{fig:experiments_failure_cases_invalid}).
		{\color{purple} TODO: do we need the visus for the failure cases? can we just put the limitations in the text? actually (b) is not a failure but a feature}
	}

	\label{fig:experiments_failure_cases}
\end{figure}


==> paper_figures/scores_over_sequence.tex <==
% !TEX root = ../paper.tex
%%
\begin{figure}
    \centering

    \input{tikz/scores_over_sequence.tikz}

    \caption{
        \textbf{Temporal Stability}:
        The figure shows the mean realism score~$S^\Real{}$ for each sample in two PandaSet sequences.
        The scores are stable over time, while the ones in sequence~91 are lower on average than in sequence~1.
        This is because sequence~91 contains the scene from the anomaly detection sample, shown in \figref{fig:experiments_anomaly_pandaset}.
    }
    \label{fig:experiments_scores_over_sequence}

\end{figure}


==> paper_tables/metrics.tex <==
% !TEX root = ../paper.tex
%%
\begin{table*}[t]
	\centering
	\caption{
		\textbf{GAN Evaluation Measures}:
		The table gives an overview on a selection of commonly used GAN evaluation measures.
		They are sorted into categories based on their operation scheme.
		The pros and cons refer to all measures within the category, though they might correspond to them in different intensity levels.
		For more information, either take a look at the examples or refer to one of these survey papers~\cite{Lucic2018NIPS,Xu2018ArXiv,Borji2019CVIU}.
	}
	\label{tab:metrics}

	\resizebox{\textwidth}{!}{%

		\begin{tabularx}{\linewidth}{l p{3cm} p{7cm} p{7cm}}
			\toprule
			Category & Examples & Pro & Con \\
			\midrule
			Qualitative Measures & \cite{Goodfellow2014NIPS,Huang2017CVPR,Zhang2017ICCV,Srivastava2017NIPS,Lin2018NIPS,Chen2016NIPS,Mathieu2016NIPS} & simple visualization required & very subjective to the observer, not usable for comparison across different work, hardly applicable to LiDAR data because humans are not good in judging point cloud quality naturally~\cite{Triess2019IV} \\
			ImageNet-based & \cite{Salimans2016NIPS,Heusel2017NIPS,Gurumurthy2017CVPR,Che2017ICLR,Zhou2018ICLR} & well established and widely used, pre-trained models available & builds on ImageNet~\cite{ImageNet2009} $\rightarrow$ no similar established dataset for LiDAR, thus not applicable to LiDAR \\
			Distribution-based & \cite{Tolstikhin2017NIPS,Gretton2012JMLR,Arora2018ICLR,Richardson2018NIPS} & successfully capture diversity and mode collapse, applicable to a variety of data types & time consuming, requires several runs over the test data, visual inspection is required \\
			Classification-based & \cite{Santurkar2018ICML,Lehmann2006,Yang2017ICLR} & every binary classifier can be adopted & requires repeated training of fresh discriminator \\
			Model Comparison & \cite{Im2016ArXiv,Olsson2018ArXiv,Zhang2018ArXiv} & evaluation of sample diversity, comparison of GAN architectures & do not consider generated output directly, very expensive in time and complexity \\
			\multirow{2}{*}{\makecell[l]{Low-Level\\Statistics}} & \cite{Zeng2017ArXiv,Khrulkov2018ICML,Wang2004,Ridgeway2015ArXiv,Karras2018ICLR} & very easy and fast to compute & specific for images, not capable to capture higher-level information \\
			\bottomrule
		\end{tabularx}

	}  % end of resize box

\end{table*}


==> suppl_figures/experiments_anomaly_patch_noise.tex <==
% !TEX root = ../paper.tex
%%
\begin{figure}
	\centering

	\begin{tabular}{lll}
		\textcolor{real_img}{\rule{2.4mm}{2.4mm}} \Real{} & \textcolor{syn_img}{\rule{2.4mm}{2.4mm}} \Syn{} & \textcolor{misc_img}{\rule{2.4mm}{2.4mm}} \Misc{}
	\end{tabular}

	\begin{subfigure}{0.48\linewidth}
		\centering

		\begin{tikzpicture}
			\begin{axis}[
				width=1.35\linewidth,
				enlargelimits=false,
				axis on top,
				axis equal image,
				ticks=none,
			]

			\addplot graphics[xmin=-60,xmax=60,ymin=-40,ymax=40] {experiments_anomaly_pandaset_patch_noise_stddev1e0.png};

			\draw[dashed] (0,0) -- (30,40);
			\draw[dashed] (0,0) -- (60,17);
			\draw[dashed] (0,0) -- (60,4);
			\draw[dashed] (0,0) -- (52,-40);

			\addplot graphics[xmin=-2.66,xmax=2.66,ymin=-1.4,ymax=1.4] {ego_vehicle_top_view_ortho.png};

			\end{axis}
		\end{tikzpicture}

		\caption{\label{fig:experiments_anomaly_patch_noise_low}Noise with $\sigma=1m$}
	\end{subfigure}%
	\hspace{4pt}%
	\begin{subfigure}{0.48\linewidth}
		\centering

		\begin{tikzpicture}
			\begin{axis}[
				width=1.35\linewidth,
				enlargelimits=false,
				axis on top,
				axis equal image,
				ticks=none,
			]

			\addplot graphics[xmin=-60,xmax=60,ymin=-40,ymax=40] {experiments_anomaly_pandaset_patch_noise_stddev8e0.png};

			\draw[dashed] (0,0) -- (-16,40);
			\draw[dashed] (0,0) -- (12,40);

			\addplot graphics[xmin=-2.66,xmax=2.66,ymin=-1.4,ymax=1.4] {ego_vehicle_top_view_ortho.png};

			\end{axis}
		\end{tikzpicture}

		\caption{\label{fig:experiments_anomaly_patch_noise_high}Noise with $\sigma=8m$}
	\end{subfigure}

	\caption{
		\textbf{Detection of sensor failures}:
		Shown are two examples where randomly selected patches of PandaSet point clouds are distorted.
		Gaussian noise with standard deviation of $\sigma$ in meters is added to the original values.
		Shown are the interpolated softmax values for all three categories.
		The metric clearly identifies the regions with the distorted patches (purple regions).
		{\color{purple} TODO: can we make one figure with real-world anomalies to save space on the caption?}
	}

	\label{fig:experiments_anomaly_patch_noise}
\end{figure}


==> suppl_figures/experiments_pandaset_gaussian_levels.tex <==
% !TEX root = ../paper.tex
%%
\begin{figure}
    \centering

    \input{tikz/pandaset_gaussian_levels.tikz}

    \caption{
        \textbf{Gaussian Distortion Levels}:
        The x-axis shows increasing values of Gaussian noise that is applied to the distance measurements of PandaSet point clouds.
        When the noise factor increases, the \Real{} score declines while the Misc score rises.
        For small standard deviations the data appears slightly more synthetic, therefore the Syn score increases slightly before declining at higher noise levels.
    }
    \label{fig:experiments_distortion_levels}

\end{figure}


==> suppl_tables/experiments_upsampling_metric_2x.tex <==
% !TEX root = ../paper.tex
%%
\begin{table}
	\centering

	\caption{
		\textbf{Metric Scores over Up-Sampling Methods}:
		This table compares five different up-sampling method and displays the \textit{Ground Truth} scores for reference.
		Here, 2~$\times$~resolution enhancement was conducted.
		We report three classical metric scores, Mean Squared Error (MSE), Mean Absolute Error (MAE), and Chamfer Distance (CD).
		These scores show the reconstruction errors between the up-sampled data and the \textit{Ground Truth} target.
		The other three scores, Misc, Real and Syn, are the mean softmax results of our metric which does not require a target.
	}

	\label{tab:experiments_upsampling_metric_2x}

	\resizebox{\linewidth}{!}{%
	\begin{tabularx}{\linewidth}{lrrrrrr}
		\toprule
		\makecell[l]{Up-Sampling\\Method} & MSE & MAE & CD & Misc & Real & Syn \\
		\midrule
		Ground Truth			& 0.00 & 0.00 &   0.0 & 0.02 & 0.69 & 0.29 \\
		Nearest Neighbor		& 0.38 & 1.83 & 122.0 & 0.01 & 0.65 & 0.34 \\
		Bilinear				& 0.88 & 0.15 &  75.2 & 0.03 & 0.65 & 0.32 \\
		$\mathcal{L}_1$-CNN	& 0.37 & 0.59 &  16.7 & 0.05 & 0.66 & 0.30 \\
		$\mathcal{L}_2$-CNN	& 0.56 & 0.69 &  16.7 & 0.13 & 0.58 & 0.29 \\
		GAN					& 0.93 & 1.46 &  76.9 & 0.16 & 0.56 & 0.28 \\
		\bottomrule
	\end{tabularx}
	}  % end of resize box

\end{table}

